Graph Neural Networks and Representation Embedding for Table Extraction in PDF Documents

Tables are widely used in several types of documents since they can bring important information in a structured way. In scientific papers, tables can sum up novel discoveries and summarize experimental results, making the research comparable and easily understandable by scholars. Several methods perform table analysis working on document images, losing useful information during the conversion from the PDF files since OCR tools can be prone to recognition errors, in particular for text inside tables. The main contribution of this work is to tackle the problem of table extraction, exploiting Graph Neural Networks. Node features are enriched with suitably designed representation embeddings. These representations help to better distinguish not only tables from the other parts of the paper, but also table cells from table headers. We experimentally evaluated the proposed approach on a new dataset obtained by merging the information provided in the PubLayNet and PubTables-1M datasets.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Response.tex <==
\
\vspace{10cm}

\newpage

\vspace{10cm}

\section*{Response  to reviewers}
\textbf{Paper}: 1484.
{\em  Graph Neural Networks and Representation Embedding for Table Extraction in PDF Documents},
A. Gemelli, E. Vivoli, and S. Marinai.\\

Dear Editor and reviewers,

We greatly appreciate the thorough and thoughtful comments provided on our submitted article. 
Overall, we agree with the comments of the referees. We made sure that each one of the reviewer's comments has been addressed carefully and the paper is revised accordingly.
In what follows the referees’ comments are in {\color{black} black} and the authors’ responses are in {\color{blue} blue}.
We will be happy to address any additional questions or concerns about the manuscript in case the paper will be accepted for publication.
\\
Sincerely, The authors. 
\vspace{-0.2cm}
\section*{Issues}
To deal with space constraints, we summarize here the issues we found in common with more than one reviewer:
\\ \ \\
\textbf{Issue 1: Grammar mistakes}
\label{issue1}
We have reread and rewritten carefully the whole paper, correcting the errors and clarifying unclear parts. In particular, sections I and II have been significantly revisited.
\\ \ \\
\textbf{Issue 2: Lack of Comparisons}
We tried to compare our method with Faster-RCNN and Mask-RCNN models pretrained on \cite{19-08-PubLayNet} \cite{19-08-TableBank}. They use mAP@[.5:.95]: this metric is not feasible for our model since we are working at token-level. We grouped PyMuPDF blocks producing object detection-like outputs. The first results appear interesting, however, given the limited time available for resubmitting this paper we were unable to obtain clear results.
Some comments are added in Section \ref{results}, with the help of Fig. \ref{fig:inference}. The only work that operates at token-level on a similar task is \cite{20-06-DocBank}. Since we had limited time to modify the paper we could not finalize a comparison with LayoutLM \cite{19-12-LayoutLM} that is left for future work. 
\\ \ \\
\textbf{Issue 3: Table Extraction}
The problem formulation was unclear, thanks for pointing out this issue. First of all, in the proposed method we are trying to do what other methods do in subsequent steps and solve TD, TSR, and TFA at once. We added Section \ref{sec:compare} to explain this point providing also some comparisons with other discussed methods. We already achieved TD and TFA: we are still dealing with the edge classification path of our model to tackle TSR.
In addition, since there are different annotations on the same source of data (in PubLayNet and PubTables-1M) we merged the datasets to bring more information into the learning process so as to create a model capable to extract as much information as possible from scientific papers.

\section*{Answers}

\subsection*{Reviewer 1:}

\begin{enumerate}

    \item Explain why GNN can extract table better \\
        {\color{blue} Tables present precise structures that, otherwise, would be lost (using CV or Language models). Insights can be found in section \ref{sec-related}}
    
    \item Give examples that the existing algorithms fail and your one can succeed \\
        {\color{blue} See Issue 2}
    
    \item Improve English \\
        {\color{blue} See Issue 1}

\end{enumerate}


\subsection*{Reviewer 2:}

\begin{enumerate}
    \item The paper applies a set of well known techniques (word embeddings, visibility graphs, message passing methods, ...etc) to solve a practical problem in document analysis. \\
    {\color{blue} We propose new embeddings for structured textual content, called \textit{representation embedding}, to solve Table Extraction (see Issue 3).}
    
    \item The paper has some weaknesses that lend itself to much room for improvement. The main reason for giving this work a weak reject is the lack of rigour in the experimentation framework, and weaknesses in the write-up, which makes the paper difficult to follow. More details below.\\
        {\color{blue} See Issue 1 and Issue 2}
    
    \item The techniques described in the paper (GNNs, word embeddings, bounding-boxes, ...etc)  have previously been applied to the problem described. In fact, in Section II.B, the authors describe many of these methods. However, it is not clear how these methods (or at least a few of them) compare to the proposed approach. If the problem being solved in these works is not the same as the one addressed here, then this was not clear in the write-up. \\
    {\color{blue} Our previous presentation of related works was not pointing out the real novelty of our proposed method. The section \ref{sec-related} has been rewritten and clarified. In addition, a table comparing features of the proposed method with other ones has been added in Section \ref{sec:compare} to clarify what we are doing.}
    
    \item The question that the reader is left with is: why do we need a model that is very similar to existing work and solves the same problem? \\
    {\color{blue} We propose a GNN model with new embeddings and edge weights to tackle the task of Table Extraction (now clarified) and Document Layout Analysis at once. Novelty comparison can be found in Table \ref{tab-compare}. Usually, tasks related to tables are carried out separately or in subsequent steps. By putting more information together we extract in a more exhaustive way scientific paper contents, crucial for research (as pointed out in \cite{20-04-AxCell}).}
    
    \item One special weakness (easily remedied) is the fact that there are no experimental results that compare the proposed model to an existing one; Or at least to a very simple baseline.
    The numbers presented in Table \ref{tab:experiment} need to be contrasted to a baseline model to have meaning.  \\
        {\color{blue} See Issue 2}
    
    \item The grammar and writing of Sections I and II need to be proofread. There are many grammatical errors that should be fixed to make the text more readable. For example "In the other hand", "documents has", "result in method improving", "in an unified way", "some table are not", ...etc are phrases that are easy to fix, but it is important to do so.\\
        {\color{blue} See Issue 1}
    
    \item In Section \ref{sec-graph}, it was very unintuitive to me why the other features added to the nodes (\% character, \% digits, ...etc) would be necessary/helpful. Any insight into what the intuition here was would be very helpful. \\
    {\color{blue} We followed the idea of \cite{19-04-TDInvoice} (better explained now in Section \ref{sec-graph}). 
    Additional ablation studies about their effectiveness were not conducted.
    }
    
    \item Section \ref{sec-repr} was unclear. What exactly are we building these patterns (header, rhombus, linear) and what are we doing with them? How do the representations in this section fit with the model architecture? \\ 
    {\color{blue} 
    The patterns (header, rhombus, linear) are used for creating the data on which representation vectors are trained with the Word2Vect approach. To train these vectors, we define three methods for \textit{visiting} tables and defining context and target elements (exhaustive explanations are given in Section \ref{sec-repr}). We use them in the GNN model as additional information for node features. By doing so, we noticed a slight improvement over table-cell and table-header F1 scores.}
     
    \item In Section \ref{sec-ours}, it is mentioned that the number of GNN layers is 4, but before then it is also mentioned that the aggregation happens only with 1-hop neighbours. These two notions seem contradictory. Please clarify. \\
    {\color{blue}The 1-hop neighbor aggregation was referred to "one layer" message passing (the formula itself is described in section \ref{sec-mess-pass}). We have rewritten Section \ref{sec-islands} where the concept was unclear and we clarified it.
    At training time, we are aggregating further information on the graph in each node by concatenating multiple GNN layers.}
    
    \item Can you explain what A, B, C, ... F represent in Table \ref{tab:experiment}? Even as it could be inferred from the table, but there is room for misunderstanding what the experiment does exactly. It would be clearer if there is a textual explanation as to what version of the model they encode. \\
    {\color{blue} We use them in Section \ref{results} to easily refer to the rows (models) that we are discussing. We added a clearer explanation in section \ref{results}, to point out each of them.}
\end{enumerate}

\subsection*{Reviewer 3:}

\begin{enumerate}
    \item Please define the task of table extraction more clearly. \\
        {\color{blue} See Issue 3}
    
    \item In addition, the definition of Table Understanding in Related Work is not exact. \\
        {\color{blue} We wanted to summarize the definition in our own words, that is why the definition was partial and wrong. It has been changed to follow the formal definitions in  \cite{21-06-Current}.}
    
    \item This work treats the single word as basic input unit. However, most OCR tools extract the bounding boxes and texts in line-level. When applying to the scanned document images, does your model can still work effectively? \\
    {\color{blue} The tool used in this work is PyMuPDF, which can extract, in addition to token-level elements, also lines' and blocks' bounding boxes. Despite the fact that we use PDFs, we also support OCR inputs. In fact, our model is agnostic to the size and the granularity of elements as long as positional information is given. However, we did not take into consideration additional experiments investigating line-level elements and embeddings.}
    
    \item The problems tackled in this work contain layout analysis and table cells/headers recognition. There are many works[1] to solve these problems separately. The comparison with other state-of-the-art methods should be provided.
    [1] Jimeno Yepes etc. ICDAR 2021 Competition on Scientific Literature Parsing. In 2021 International Conference on Document Analysis and Recognition (ICDAR). IEEE https://arxiv.org/abs/2106.14616v1\\
    {\color{blue} An exhaustive answer to comparisons is given in Issue 2. We were not  able to directly compare with DAVAR-Lab-OCR models, but their work has been taken into consideration in Section \ref{ref:SOA-tables} and Section \ref{sec:compare}.}
    
    \item Compared with detection-based method, the advantages of this method should be explained. \\
    {\color{blue} Using only detection-based methods would end in a partial result: as shown in Section \ref{ref:SOA-tables} the table structure is inferred along with Table Detection using heuristics or in two steps involving two different networks. A GNN already brings the structure into the training process (using edges between elements) and applying edge classification would tackle TD and TSR at once. Also, for TFA, the recognition of Headers is really connected to the structure, since their position in tables has a precise meaning. Issues 2 and 3 along with rewritten Introduction and Related Works sections, should clarify more this answer.}
\end{enumerate}

\section*{Summary}
The elements employed in our work are not totally new. Anyway, we proposed a new representation embedding and, along with ablation studies and comparison with Spacy and SciBERT, we have shown its effectiveness for Table Extraction and Document Layout Analysis. 

To the best of our knowledge, we are the first ones who addressed Table Extraction with an end-to-end approach to accomplish this task at once. In fact, in the literature, tables are firstly detected, and only then their structure is analyzed. We still need to complete the experiments, but the method based on GNNs is expected to be capable to learn the structure tables. Anyway, we have already addressed the Functional Analysis finding table headers.

Our primary aim is also to extract as much information as possible from the scientific papers, such as captions, titles, and so on. In order to tackle both tasks (DLA and TE) together, we needed a dataset containing all the necessary: That is why we merged both PubTables-1m and PubLayNethoping. This dataset will also be useful for other researchers to move forward in this direction. 

